Optimality Implies Kernel Sum Classifiers are Statistically Efficient

We propose a novel combination of optimization tools with learning theory bounds in order to analyze the sample complexity of optimal kernel sum classifiers. This contrasts the typical learning theoretic results which hold for all (potentially suboptimal) classifiers. Our work also justifies assumptions made in prior work on multiple kernel learning. As a byproduct of our analysis, we also provide a new form of Rademacher complexity for hypothesis classes containing only optimal classifiers.

==> app-rademacher-learn-kernel.tex <==
\todo{DO NOT INCLUDE THIS FILE UNLESS THE UNION BOUND PROOF IS ACTUALLY USEFULL}

\section{Proof of Learning Kernels (\theoremref{...})}
\begin{reptheorem}{...}
Fix \(n > 0\), \(\delta\in(0,1)\), and \(\gamma\in(0,1)\).
Define the \(\gamma\)-Lipschitz Loss function
\[
	\psi(x)\defeq
	\begin{cases}
		1 & x < 0 \\
		1-\frac x\gamma & 0 \leq x \leq \gamma \\
		0 & x > \gamma
	\end{cases}
\]
Sample a dataset \(\cS\sim\cD^n\).
Let \(k_1,\ldots,k_m\) be kernel functions.
Define \(k_{_\cP}(\cdot,\cdot)\defeq\sum_{t\in\cP}k_t(\cdot,\cdot)\) for some \(\cP\subseteq[m]\).
Compute the labeled kernel matrices \(\mKt_1,\ldots,\mKt_m\) and \(\mKt_{_\cP}\).
Find the corresponding Dual SVM solutions \(\valpha_1,\ldots,\valpha_m\) and \(\valpha_{_\cP}\).
Assume \(k_t(\vx_i,\vx_i) \leq R^2\) and \(\valpha_t^\intercal\mKt_t\valpha_t\leq B^2\) for all \(t\in[m]\) and \(i\in[n]\).
Define
\[
	\eps \defeq \frac{BR}{\gamma} \sqrt{12e\eta_0 m^{^{1-\log_2(\nicefrac{3}{2})}} \ceil{\ln(m)}} + \left(\frac 8\gamma + 1\right) \sqrt{\frac{\ln(4m/\delta)}{2}}
\]
where \(\eta_0=\frac{23}{22}\).
Then with probability \(1-\delta\), for all \(f\in\cF_{_\cP}\),
\[
	\Pr_{(\vx,y)\sim\cD}[yf(x)\leq0]
	\leq
	\frac1n\sum_{i=1}^{n}\psi(y_i f(\vx_i)) + \frac{\eps}{\sqrt n}
\]
\end{reptheorem}
\begin{proof}
For visual clarity, let \(\risk_n(f)\defeq \Pr_{(\vx,y)\sim\cD}[yf(x)\leq0] - \frac1n\sum_{i=1}^{n}\psi(y_i f(\vx_i))\).
So, we just need to show that \(\risk_n(f)\leq\frac{\eps}{\sqrt{n}}\) for all \(f\in\cF_{_\cP}\) with high probability.

Recall \theoremref{bartlett-lipschitz-risk}.
We instantiate this theorem on \(\cF_s\).
That is, for all \(\delta_0\in(0,1)\),
\[
	\Pr\left[\exists f \in \cF_s, \risk\nolimits_n(f) \geq \frac2\gamma \hat\fR_\cS(\cF_{_\cP}) + \left(\frac8\gamma + 1\right) \sqrt{\frac{\ln(4/\delta_0)}{n}}\right] \leq \delta_0
\]
We will take \(\delta_0=\nicefrac{\delta}{m}\).
Also recall \theoremref{rademacher-subset-bound}.
Subsituting these into the probability above,
\[
	\Pr\left[\exists f \in \cF_s, \risk\nolimits_n(f) \geq \frac{\eps}{\sqrt n}\right] \leq \frac{\delta}{m}
\]

Now, we union bound over all possible \(\cF_s\):
\begin{align*}
	\Pr\left[\exists f \in \cF_{_\cP}, \risk\nolimits_n(f)\geq \frac{\eps}{\sqrt{n}}\right]
	&= \Pr\left[\exists s\in[m], \exists f \in \cF_s, \risk\nolimits_n(f)\geq \frac{\eps}{\sqrt{n}} \right] \\
	&\leq \sum_{s=1}^{m} \Pr\left[\exists f \in \cF_s, \risk\nolimits_n(f)\geq \frac{\eps}{\sqrt{n}} \right] \\
	&\leq \sum_{s=1}^{m} \frac{\delta}{m} \\
	&= \delta
\end{align*}
This completes the proof.
\end{proof}

